Geometry of abstraction in quantum computation

Quantum algorithms are sequences of abstract operations, performed on non-existent computers. They are in obvious need of categorical semantics. We present some steps in this direction, following earlier contributions of Abramsky, Coecke and Selinger. In particular, we analyze function abstraction in quantum computation, which turns out to characterize its classical interfaces. Some quantum algorithms provide feasible solutions of important hard problems, such as factoring and discrete log (which are the building blocks of modern cryptography). It is of a great practical interest to precisely characterize the computational resources needed to execute such quantum algorithms. There are many ideas how to build a quantum computer. Can we prove some necessary conditions? Categorical semantics help with such questions. We show how to implement an important family of quantum algorithms using just abelian groups and relations.

==> PIC/DagAbs.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Thu Apr 03 23:09:04 BST 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="11" x-max="56" y-min="-5" y-max="22" auto-bounding="true">
%<multicurve arrow-tbar-width-minimum= "0.15"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(21,20);(21,20);(39,20);(39,20)"
%	 />
%<multicurve arrow-tbar-width-minimum= "0.15"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(21,0);(21,0);(39,0);(39,0)"
%	 />
%<multicurve arrow-tbar-width-minimum= "0.15"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(44,17);(44,17);(44,2);(44,2)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(56,-5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 arrow-tbar-width-minimum= "0.15"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-linewidth-scale= "2"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(19,20)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$X\otimes B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,0)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$X\otimes X\otimes B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,0)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$X\otimes A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,20)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$X\otimes X\otimes A$
%</text>
%<multicurve arrow-tbar-width-minimum= "0.15"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(12,17);(12,17);(12,2);(12,2)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,10)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle \nabla\otimes A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(11,10)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle \Delta \otimes B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,22)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes \left(\kappa x.\varphi(x)\right)^\ddag $
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,-2)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes \kappa x.\varphi(x)^\ddag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(56,22)
\psline[tbarsize=0.15 5]{->}(21,20)(39,20)
\psline[tbarsize=0.15 5]{->}(21,0)(39,0)
\psline[tbarsize=0.15 5]{->}(44,17)(44,2)
\rput(56,-5){}
\rput[r](19,20){$X\otimes B$}
\rput[r](20,0){$X\otimes X\otimes B$}
\rput[l](40,0){$X\otimes A$}
\rput[l](40,20){$X\otimes X\otimes A$}
\psline[tbarsize=0.15 5]{->}(12,17)(12,2)
\rput[l](45,10){$\scriptstyle \nabla\otimes A$}
\rput[r](11,10){$\scriptstyle \Delta \otimes B$}
\rput(30,22){$\scriptstyle X\otimes \left(\kappa x.\varphi(x)\right)^\ddag $}
\rput(30,-2){$\scriptstyle X\otimes \kappa x.\varphi(x)^\ddag$}
\end{pspicture}


==> PIC/DagKappa.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Oct 10 17:50:49 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="50" y-min="-6" y-max="27" auto-bounding="true">
%<text arrow-tbar-width-linewidth-scale= "2"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40.75,-6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 arrow-tbar-width-minimum= "0.15"
%	 fill-style= "none"
%	 left-arrow= "t-bar-flushed"
%	 >
%
%</text>
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(45,20);(45,20);(45,25);(45,25)"
%	 />
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(35,25);(35,25);(35,20);(35,20)"
%	 />
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(45,10);(45,10);(45,5);(45,5)"
%	 />
%<parallelogram p3= "(50,10)"
%	 stroke-width= "0.1"
%	 p1= "(30,20)"
%	 right-arrow= "head"
%	 p2= "(50,20)"
%	 fill-style= "solid"
%	 fill-color= "#ffff99"
%	 />
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(15,20);(15,20);(15,25);(15,25)"
%	 />
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(5,10);(5,10);(5,5);(5,5)"
%	 />
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(15,10);(15,10);(15,5);(15,5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(46,23)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 >
%$A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16,7)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 >
%$B$
%</text>
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(7.5,5.5);(7.5,5.5);(5,3);(5,3);(5,3);(2.5,5.5);
%	(2.5,5.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$=$
%</text>
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(32.5,24.5);(32.5,24.5);(35,27);(35,27);(35,27);(37.5,24.5);
%	(37.5,24.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,14.38)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\left(\kappa x.\varphi(x)\right)^\ddag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(46,7)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$B$
%</text>
%<parallelogram p3= "(20,10)"
%	 stroke-width= "0.1"
%	 p1= "(0,20)"
%	 right-arrow= "head"
%	 p2= "(20,20)"
%	 fill-style= "solid"
%	 fill-color= "#ffff99"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16,23)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 >
%$A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,14.38)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\kappa x.\varphi(x)^\ddag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(50,27)
\rput(40.75,-6){}
\psline[linewidth=0.15](45,20)(45,25)
\psline[linewidth=0.15](35,25)(35,20)
\psline[linewidth=0.15](45,10)(45,5)
\newrgbcolor{userFillColour}{1 1 0.6}
\pspolygon[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid](30,20)(50,20)(50,10)(30,10)
\psline[linewidth=0.15](15,20)(15,25)
\psline[linewidth=0.15](5,10)(5,5)
\psline[linewidth=0.15](15,10)(15,5)
\rput[l](46,23){$A$}
\rput[l](16,7){$B$}
\psline[linewidth=0.05,fillstyle=solid](7.5,5.5)
(5,3)(2.5,5.5)
\rput(25,15){$=$}
\psline[linewidth=0.05,fillstyle=solid](32.5,24.5)
(35,27)(37.5,24.5)
\rput(40,14.38){$\left(\kappa x.\varphi(x)\right)^\ddag$}
\rput[l](46,7){$B$}
\newrgbcolor{userFillColour}{1 1 0.6}
\pspolygon[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid](0,20)(20,20)(20,10)(0,10)
\rput[l](16,23){$A$}
\rput(10,14.38){$\kappa x.\varphi(x)^\ddag$}
\rput(7.5,15){}
\end{pspicture}


==> PIC/Frob2.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Thu Apr 10 21:48:15 PDT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="8.38" x-max="55.38" y-min="1" y-max="28" auto-bounding="true">
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(52,27);(52,27);(52,1);(52,1)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(39.5,14)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(27.51,10.92);(27.51,10.92);(27.5,28);(27.5,28)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(15.5,24.71);(15.5,24.71);(15.5,21);(15.5,21)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(11.5,1);(11.5,1);(11.5,17);(11.5,17)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(17.5,11);(17.5,11);(29.5,11);(29.5,11);(29.5,11);(26.5,7);
%	(26.5,7);(26.5,7);(20.5,7);(20.5,7);(20.5,7);(17.5,11)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(23.5,7);(23.5,7);(23.45,2.13);(23.45,2.13)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(21.5,17);(21.5,17);(9.5,17);(9.5,17);(9.5,17);(12.5,21);
%	(12.5,21);(12.5,21);(18.5,21);(18.5,21);(18.5,21);(21.5,17)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.5,19)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monoid$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(19.5,11);(19.5,11);(19.5,17);(19.5,17)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.5,9)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonoid$
%</text>
%<multicurve fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(12.62,22.77);(12.62,22.77);(15.62,26.77);(15.62,26.77);(15.62,26.77);(18.62,22.77);
%	(18.62,22.77);(18.62,22.77);(12.62,22.77);(12.62,22.77)"
%	 />
%<multicurve fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(26.55,5.09);(26.55,5.09);(23.55,1.09);(23.55,1.09);(23.55,1.09);(20.55,5.09);
%	(20.55,5.09);(20.55,5.09);(26.55,5.09);(26.55,5.09)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.54,3.82)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.59,23.82)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(53.12,13.75)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\obj$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(14.38,5);(14.38,5);(11.38,1);(11.38,1);(11.38,1);(8.38,5);
%	(8.38,5);(8.38,5);(14.38,5);(14.38,5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(55.38,5);(55.38,5);(52.38,1);(52.38,1);(52.38,1);(49.38,5);
%	(49.38,5);(49.38,5);(55.38,5);(55.38,5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(55.38,28)
\psline[linewidth=0.22](52,27)(52,1)
\rput(39.5,14){$\eqls$}
\psline[linewidth=0.22](27.51,10.92)(27.5,28)
\psline[linewidth=0.22](15.5,24.71)(15.5,21)
\psline[linewidth=0.22](11.5,1)(11.5,17)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](17.5,11)
(29.5,11)
(26.5,7)
(20.5,7)(17.5,11)
\psline[linewidth=0.22](23.5,7)(23.45,2.13)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](21.5,17)
(9.5,17)
(12.5,21)
(18.5,21)(21.5,17)
\rput(15.5,19){$\monoid$}
\psline[linewidth=0.22](19.5,11)(19.5,17)
\rput(23.5,9){$\comonoid$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](12.62,22.77)
(15.62,26.77)
(18.62,22.77)(12.62,22.77)
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](26.55,5.09)
(23.55,1.09)
(20.55,5.09)(26.55,5.09)
\rput(23.54,3.82){$\monunit$}
\rput(15.59,23.82){$\comonunit$}
\rput[l](53.12,13.75){$\obj$}
\psline[linewidth=0.22,fillstyle=solid](14.38,5)
(11.38,1)
(8.38,5)(14.38,5)
\psline[linewidth=0.22,fillstyle=solid](55.38,5)
(52.38,1)
(49.38,5)(55.38,5)
\end{pspicture}


==> PIC/Lambek-old.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue May 31 12:33:44 CEST 2011
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="7" x-max="53" y-min="1" y-max="14" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(32,1)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\blah$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(32,13)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\picSetxBlahh$
%</text>
%<ellipse fill-style= "none"
%	 p3= "(31,4)"
%	 p2= "(31,11)"
%	 right-arrow= "head"
%	 p1= "(28,11)"
%	 closure= "open"
%	 angle-end= "251.57"
%	 angle-start= "108.43"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(31.5,11)"
%	 p2= "(31.5,4)"
%	 right-arrow= "head"
%	 p1= "(34.5,4)"
%	 closure= "open"
%	 angle-end= "251.57"
%	 angle-start= "108.43"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(36,7)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<multicurve fill-style= "none"
%	 right-arrow= "head"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 points= "(53,11);(53,11);(53,4);(53,4)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "head"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 points= "(7,4);(7,4);(7,11);(7,11)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(53,14)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(53,2)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(7,14)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(7,2)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(53,14)
\rput(32,1){$\blah$}
\rput(32,13){$\picSetxBlahh$}
\rput{90}(29.5,7.5){\psellipticarc[]{->}(0,0)(3.5,-1.5){-161.57}{-18.43}}
\rput{90}(33,7.5){\psellipticarc[]{->}(0,0)(3.5,-1.5){18.43}{161.57}}
\rput(36,7){}
\psline[tbarsize=0.15 5]{|*->}(53,11)(53,4)
\psline[tbarsize=0.15 5]{|*->}(7,4)(7,11)
\rput(53,14){$\one$}
\rput(53,2){$\two$}
\rput(7,14){$\three$}
\rput(7,2){$\four$}
\end{pspicture}


==> PIC/Mes-b1.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Tue Jul 07 08:16:18 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="4.75" x-max="53.62" y-min="0.75" y-max="27.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(51.88,10.88);(51.88,10.88);(51.88,26.88);(51.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(39.74,27);(39.74,27);(39.74,21);(39.74,21)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(35.74,1);(35.74,1);(35.74,17);(35.74,17)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(41.74,11);(41.74,11);(53.62,11);(53.62,11);(53.62,11);(53.62,7);
%	(53.62,7);(53.62,7);(45.62,7);(45.62,7);(45.62,7);(41.74,11)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(51.88,6.88);(51.88,6.88);(51.88,0.88);(51.88,0.88)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(45.74,17);(45.74,17);(33.74,17);(33.74,17);(33.74,17);(37.62,21);
%	(37.62,21);(37.62,21);(41.62,21);(41.62,21);(41.62,21);(45.74,17)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(43.74,11);(43.74,11);(43.74,17);(43.74,17)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(39.62,19)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\monoid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.75,9.38)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\coalgebra$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,25)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,1.88)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,2.5)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(39.38,25)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(14.87,17.13);(14.87,17.13);(14.87,11.13);(14.87,11.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(6.37,1.13);(6.37,1.13);(6.37,7.13);(6.37,7.13)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(16.87,7.13);(16.87,7.13);(4.87,7.13);(4.87,7.13);(4.87,7.13);(9.87,11.13);
%	(9.87,11.13);(9.87,11.13);(16.87,11.13);(16.87,11.13);(16.87,11.13);(16.87,7.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(14.87,0.75);(14.87,0.75);(14.87,7.13);(14.87,7.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(14.87,21);(14.87,21);(14.87,27);(14.87,27)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(4.75,21.13);(4.75,21.13);(16.63,21.13);(16.63,21.13);(16.63,21.13);(16.63,17.13);
%	(16.63,17.13);(16.63,17.13);(8.63,17.13);(8.63,17.13);(8.63,17.13);(4.75,21.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(6.75,21.13);(6.75,21.13);(6.75,27.13);(6.75,27.13)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(11.87,9.13)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(11.75,9.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\algebra$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(11.75,19.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\coalgebra$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,1.88)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,24.38)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5.62,1.88)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(6.25,24.38)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,13.75)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\eqls$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(53.62,27.13)
\psline[linewidth=0.22](51.88,10.88)(51.88,26.88)
\psline[linewidth=0.22](39.74,27)(39.74,21)
\psline[linewidth=0.22](35.74,1)(35.74,17)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](41.74,11)
(53.62,11)
(53.62,7)
(45.62,7)(41.74,11)
\psline[linewidth=0.22](51.88,6.88)(51.88,0.88)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](45.74,17)
(33.74,17)
(37.62,21)
(41.62,21)(45.74,17)
\psline[linewidth=0.22](43.74,11)(43.74,17)
\rput(39.62,19){$\monoid$}
\rput(48.75,9.38){$\coalgebra$}
\rput[l](52.5,25){$\objA$}
\rput[l](52.5,1.88){$\objA$}
\rput[r](35,2.5){$\objX$}
\rput[r](39.38,25){$\objX$}
\psline[linewidth=0.22](14.87,17.13)(14.87,11.13)
\psline[linewidth=0.22](6.37,1.13)(6.37,7.13)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](16.87,7.13)
(4.87,7.13)
(9.87,11.13)
(16.87,11.13)(16.87,7.13)
\psline[linewidth=0.22](14.87,0.75)(14.87,7.13)
\psline[linewidth=0.22](14.87,21)(14.87,27)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](4.75,21.13)
(16.63,21.13)
(16.63,17.13)
(8.63,17.13)(4.75,21.13)
\psline[linewidth=0.22](6.75,21.13)(6.75,27.13)
\rput(11.87,9.13){}
\rput(11.75,9.5){$\algebra$}
\rput(11.75,19.5){$\coalgebra$}
\rput[l](16.25,1.88){$\objA$}
\rput[l](16.25,24.38){$\objA$}
\rput[r](5.62,1.88){$\objX$}
\rput[r](6.25,24.38){$\objX$}
\rput(25,13.75){$\eqls$}
\end{pspicture}


==> PIC/Mes-b2.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Tue Jul 07 08:08:21 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.88" x-max="51.87" y-min="0.75" y-max="27.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(4.88,11);(4.88,11);(4.88,27);(4.88,27)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(21.88,27);(21.88,27);(21.88,21);(21.88,21)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(13.38,11);(13.38,11);(13.38,17);(13.38,17)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(2.88,11);(2.88,11);(14.88,11);(14.88,11);(14.88,11);(10.88,7);
%	(10.88,7);(10.88,7);(6.88,7);(6.88,7);(6.88,7);(2.88,11)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(8.88,7);(8.88,7);(8.88,1);(8.88,1)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(23.88,17);(23.88,17);(11.88,17);(11.88,17);(11.88,17);(16.88,21);
%	(16.88,21);(16.88,21);(23.88,21);(23.88,21);(23.88,21);(23.88,17)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(21.88,1);(21.88,1);(21.88,17);(21.88,17)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,9)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\comonoid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.25,14.38)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.88,19)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.76,19.38)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\algebra$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(22.5,2.5)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.12,25)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,1.88)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(4.38,25)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(49.87,17.13);(49.87,17.13);(49.87,11.13);(49.87,11.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(41.37,1.13);(41.37,1.13);(41.37,7.13);(41.37,7.13)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(51.87,7.13);(51.87,7.13);(39.87,7.13);(39.87,7.13);(39.87,7.13);(44.87,11.13);
%	(44.87,11.13);(44.87,11.13);(51.87,11.13);(51.87,11.13);(51.87,11.13);(51.87,7.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(49.87,0.75);(49.87,0.75);(49.87,7.13);(49.87,7.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(49.87,21);(49.87,21);(49.87,27);(49.87,27)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "head"
%	 fill-color= "#ffff66"
%	 stroke-width= "0.22"
%	 points= "(39.75,21.13);(39.75,21.13);(51.63,21.13);(51.63,21.13);(51.63,21.13);(51.63,17.13);
%	(51.63,17.13);(51.63,17.13);(43.63,17.13);(43.63,17.13);(43.63,17.13);(39.75,21.13)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.22"
%	 points= "(41.75,21.13);(41.75,21.13);(41.75,27.13);(41.75,27.13)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(46.87,9.13)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(46.75,9.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\algebra$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(46.75,19.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\coalgebra$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.25,1.88)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.25,24.38)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\objA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40.62,1.88)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(41.25,24.38)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\objX$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(51.87,27.13)
\psline[linewidth=0.22](4.88,11)(4.88,27)
\psline[linewidth=0.22](21.88,27)(21.88,21)
\psline[linewidth=0.22](13.38,11)(13.38,17)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](2.88,11)
(14.88,11)
(10.88,7)
(6.88,7)(2.88,11)
\psline[linewidth=0.22](8.88,7)(8.88,1)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](23.88,17)
(11.88,17)
(16.88,21)
(23.88,21)(23.88,17)
\psline[linewidth=0.22](21.88,1)(21.88,17)
\rput(9.38,9){$\comonoid$}
\rput(31.25,14.38){$\eqls$}
\rput(18.88,19){}
\rput(18.76,19.38){$\algebra$}
\rput[l](22.5,2.5){$\objA$}
\rput[l](23.12,25){$\objA$}
\rput[r](8.12,1.88){$\objX$}
\rput[r](4.38,25){$\objX$}
\psline[linewidth=0.22](49.87,17.13)(49.87,11.13)
\psline[linewidth=0.22](41.37,1.13)(41.37,7.13)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](51.87,7.13)
(39.87,7.13)
(44.87,11.13)
(51.87,11.13)(51.87,7.13)
\psline[linewidth=0.22](49.87,0.75)(49.87,7.13)
\psline[linewidth=0.22](49.87,21)(49.87,27)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](39.75,21.13)
(51.63,21.13)
(51.63,17.13)
(43.63,17.13)(39.75,21.13)
\psline[linewidth=0.22](41.75,21.13)(41.75,27.13)
\rput(46.87,9.13){}
\rput(46.75,9.5){$\algebra$}
\rput(46.75,19.5){$\coalgebra$}
\rput[l](51.25,1.88){$\objA$}
\rput[l](51.25,24.38){$\objA$}
\rput[r](40.62,1.88){$\objX$}
\rput[r](41.25,24.38){$\objX$}
\end{pspicture}


==> PIC/Prog-2.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Wed Mar 12 19:00:02 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2" x-max="75.12" y-min="0" y-max="60" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\Clas$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\Quant$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,20)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\Meas$
%</text>
%<multicurve right-arrow= "head"
%	 arrow-global-scale-length= "1.5"
%	 arrow-global-scale-width= "1.3"
%	 fill-style= "none"
%	 points= "(20,56);(20,56);(20,43);(20,43)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,40);(20,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,39);(20,39);(20,39);(20,39)"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-global-scale-length= "1.5"
%	 left-arrow= "reverse-head"
%	 arrow-global-scale-width= "1.3"
%	 fill-style= "none"
%	 points= "(20,37);(20,37);(20,23);(20,23)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,50)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\keto$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,30)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\meso$
%</text>
%<multicurve right-arrow= "head"
%	 arrow-global-scale-length= "1.5"
%	 arrow-global-scale-width= "1.3"
%	 fill-style= "none"
%	 points= "(20,16);(20,16);(20,3);(20,3)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,0)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\Classs$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,34)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%\superposition
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-2,26)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%\entanglement
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.12,40)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\KL$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.12,20)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\EM$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.12,60)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\EX$
%</text>
%<circle stroke-color= "#ff3333"
%	 closure= "open"
%	 p3= "(10.62,40)"
%	 p1= "(2.33,28.76)"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 p2= "(4.33,36.76)"
%	 />
%<circle stroke-color= "#ff3333"
%	 closure= "open"
%	 p3= "(37.09,35.62)"
%	 right-arrow= "head"
%	 p1= "(28.75,40)"
%	 fill-style= "none"
%	 p2= "(34.09,38.62)"
%	 />
%<circle stroke-color= "#ff3333"
%	 closure= "open"
%	 p3= "(28.75,20)"
%	 p1= "(38.7,31.44)"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 p2= "(36.82,24.57)"
%	 />
%<circle stroke-color= "#ff3333"
%	 closure= "open"
%	 p3= "(10.62,20)"
%	 right-arrow= "head"
%	 p1= "(3.75,24.38)"
%	 fill-style= "none"
%	 p2= "(6.88,21.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(21.88,10)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\forget$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(75.12,60)
\rput(20,60){}
\rput(20,60){$\Clas$}
\rput(20,40){$\Quant$}
\rput(20,20){$\Meas$}
\psline[arrowscale=1.3 1.5]{->}(20,56)(20,43)
\psbezier(20,40)(20,40)(20,40)(20,40)
\psbezier(20,39)(20,39)(20,39)(20,39)
\psline[arrowscale=1.3 1.5]{>->}(20,37)(20,23)
\rput[l](22,50){$\keto$}
\rput[l](22,30){$\meso$}
\psline[arrowscale=1.3 1.5]{->}(20,16)(20,3)
\rput(20,0){$\Classs$}
\rput[r](45,34){\superposition}
\rput[l](-2,26){\entanglement}
\rput[r](75.12,40){$\KL$}
\rput[r](75.12,20){$\EM$}
\rput[r](75.12,60){$\EX$}
\newrgbcolor{userLineColour}{1 0.2 0.2}
\rput{0}(11.41,30.74){\psellipticarc[linecolor=userLineColour]{<-}(0,0)(9.29,9.29){94.83}{192.31}}
\newrgbcolor{userLineColour}{1 0.2 0.2}
\rput{0}(29.21,30.73){\psellipticarc[linecolor=userLineColour]{->}(0,0)(9.28,9.28){31.78}{92.82}}
\newrgbcolor{userLineColour}{1 0.2 0.2}
\rput{0}(28.04,30.67){\psellipticarc[linecolor=userLineColour]{<-}(0,0)(10.69,10.69){-86.18}{4.15}}
\newrgbcolor{userLineColour}{1 0.2 0.2}
\rput{0}(11.56,29.06){\psellipticarc[linecolor=userLineColour]{->}(0,0)(9.11,9.11){-149.04}{-95.91}}
\rput[l](21.88,10){$\forget$}
\end{pspicture}


==> PIC/ProofCD.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Sat Jan 10 10:31:02 PST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1" x-max="63" y-min="1" y-max="21.25" auto-bounding="true">
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(38.5,1);(38.5,1);(38.25,11.88);(38.25,11.88)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(41.38,5);(41.38,5);(38.38,1);(38.38,1);(38.38,1);(35.38,5);
%	(35.38,5);(35.38,5);(41.38,5);(41.38,5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(35.12,20);(35.12,20);(35.12,12.5);(35.12,12.5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(63,5);(63,5);(60,1);(60,1);(60,1);(57,5);
%	(57,5);(57,5);(63,5);(63,5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50.75,11.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(32.12,17.25);(32.12,17.25);(35.12,21.25);(35.12,21.25);(35.12,21.25);(38.12,17.25);
%	(38.12,17.25);(38.12,17.25);(32.12,17.25);(32.12,17.25)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(4,21);(4,21);(4,1);(4,1)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(7,5);(7,5);(4,1);(4,1);(4,1);(1,5);
%	(1,5);(1,5);(7,5);(7,5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(14,18);(14,18);(14,1);(14,1)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(17,5);(17,5);(14,1);(14,1);(14,1);(11,5);
%	(11,5);(11,5);(17,5);(17,5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(1,17);(1,17);(4,21);(4,21);(4,21);(7,17);
%	(7,17);(7,17);(1,17);(1,17)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(23,11)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(60.12,18.12);(60.12,18.12);(60.12,1.25);(60.12,1.25)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(42,18.12);(42,18.12);(42,12.5);(42,12.5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 right-arrow= "head"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(32.38,12.75);(32.38,12.75);(44.38,12.75);(44.38,12.75);(44.38,12.75);(41.38,8.75);
%	(41.38,8.75);(41.38,8.75);(35.38,8.75);(35.38,8.75);(35.38,8.75);(32.38,12.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(63,21.25)
\psline[linewidth=0.22](38.5,1)(38.25,11.88)
\psline[linewidth=0.22,fillstyle=solid](41.38,5)
(38.38,1)
(35.38,5)(41.38,5)
\psline[linewidth=0.22](35.12,20)(35.12,12.5)
\psline[linewidth=0.22,fillstyle=solid](63,5)
(60,1)
(57,5)(63,5)
\rput(50.75,11.25){$\eqls$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](32.12,17.25)
(35.12,21.25)
(38.12,17.25)(32.12,17.25)
\psline[linewidth=0.22](4,21)(4,1)
\psline[linewidth=0.22,fillstyle=solid](7,5)
(4,1)
(1,5)(7,5)
\psline[linewidth=0.22](14,18)(14,1)
\psline[linewidth=0.22,fillstyle=solid](17,5)
(14,1)
(11,5)(17,5)
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](1,17)
(4,21)
(7,17)(1,17)
\rput(23,11){$\eqls$}
\psline[linewidth=0.22](60.12,18.12)(60.12,1.25)
\psline[linewidth=0.22](42,18.12)(42,12.5)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](32.38,12.75)
(44.38,12.75)
(41.38,8.75)
(35.38,8.75)(32.38,12.75)
\end{pspicture}


==> PIC/Simon-4.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Tue Mar 11 17:50:27 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="100" y-min="10" y-max="50.62" auto-bounding="true">
%<parallelogram stroke-width= "0.15"
%	 p3= "(70.91,10)"
%	 p1= "(30,50.62)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(30,10)"
%	 />
%<multicurve stroke-width= "0.32"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(80,45);(80,45)"
%	 />
%<multicurve stroke-width= "0.32"
%	 fill-style= "none"
%	 points= "(0,15);(0,15);(100,15);(100,15)"
%	 />
%<ellipse closure= "open"
%	 p3= "(49.63,43.98)"
%	 p1= "(51.62,46.02)"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 p2= "(51.62,43.98)"
%	 angle-start= "0"
%	 />
%<ellipse stroke-width= "0.35"
%	 closure= "open"
%	 p3= "(48.58,12.97)"
%	 p1= "(52.67,17.03)"
%	 angle-end= "0"
%	 fill-style= "none"
%	 p2= "(52.67,12.97)"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(50.62,16.88);(50.62,16.88);(50.62,13.12);(50.62,13.12)"
%	 />
%<parallelogram p3= "(45.58,24.62)"
%	 p1= "(55.79,34.76)"
%	 fill-style= "none"
%	 p2= "(55.79,24.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.62,45);(50.62,45);(50.68,34.76);(50.68,34.76)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.68,24.62);(50.68,24.62);(50.62,16.88);(50.62,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(36.36,34.76)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50.62,30)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle f$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(36.88,23.12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U_f$
%</text>
%<parallelogram stroke-width= "0.15"
%	 p3= "(20,40)"
%	 p1= "(10,50)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(10,40)"
%	 />
%<parallelogram stroke-width= "0.15"
%	 p3= "(90,40)"
%	 p1= "(80,50)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(0,45);(0,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,45);(10,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(90,45);(90,45)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,45)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$H^{\otimes m}$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,45)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$H^{\otimes m}$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(36,12.38)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,13)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |y\rangle$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,47)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |x\rangle$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(76,47)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |x\rangle$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(73,13)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |f(x)\oplus y\rangle$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(76,47)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,47)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |z\rangle$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,37)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |x\rangle = \sum_z (-1)^{x\cdot z}|z\rangle $
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,47)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |z\rangle$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,37)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle |z\rangle = \sum_x (-1)^{z\cdot x}|x\rangle$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(100,50.62)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](30,50.62)(30,10)(70.91,10)(70.91,50.62)
\psline[linewidth=0.32](20,45)(80,45)
\psline[linewidth=0.32](0,15)(100,15)
\rput{90}(50.62,45){\psellipse[fillstyle=solid](0,0)(1.02,-0.99)}
\rput{-0}(50.62,15){\psellipse[linewidth=0.35](0,0)(2.04,-2.03)}
\psline[linewidth=0.35](50.62,16.88)(50.62,13.12)
\pspolygon[](55.79,34.76)(55.79,24.62)(45.58,24.62)(45.58,34.76)
\psline(50.62,45)(50.68,34.76)
\psline(50.68,24.62)(50.62,16.88)
\rput(36.36,34.76){}
\rput(50.62,30){$\scriptstyle f$}
\rput(36.88,23.12){$U_f$}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](10,50)(10,40)(20,40)(20,50)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](80,50)(80,40)(90,40)(90,50)
\psline(10,45)(0,45)
\psbezier(10,45)(10,45)(10,45)(10,45)
\psline(100,45)(90,45)
\rput(15,45){$H^{\otimes m}$}
\rput(85,45){$H^{\otimes m}$}
\rput(36,12.38){}
\rput(24,13){$\scriptstyle |y\rangle$}
\rput(24,47){$\scriptstyle |x\rangle$}
\rput(76,47){$\scriptstyle |x\rangle$}
\rput[l](73,13){$\scriptstyle |f(x)\oplus y\rangle$}
\rput(76,47){}
\rput(5,47){$\scriptstyle |z\rangle$}
\rput(85,37){$\scriptstyle |x\rangle = \sum_z (-1)^{x\cdot z}|z\rangle $}
\rput(95,47){$\scriptstyle |z\rangle$}
\rput(15,37){$\scriptstyle |z\rangle = \sum_x (-1)^{z\cdot x}|x\rangle$}
\end{pspicture}


==> PIC/geometry-1.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Fri Jan 02 16:18:29 PST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="6.4" x-max="71.8" y-min="5.6" y-max="47.2" auto-bounding="true">
%<multicurve stroke-width= "0.1"
%	 fill-style= "solid"
%	 points= "(6.4,9.6);(6.4,9.6);(12.8,9.6);(12.8,9.6);(12.8,9.6);(9.6,6.4);
%	(9.6,6.4);(9.6,6.4);(6.4,9.6);(6.4,9.6);(6.4,9.6);(6.4,9.6);
%	(6.4,9.6)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(14.4,9.6);(14.4,9.6);(24,9.6);(24,9.6);(24,9.6);(19.2,6.4);
%	(19.2,6.4);(19.2,6.4);(14.4,9.6);(14.4,9.6);(14.4,9.6);(14.4,9.6);
%	(14.4,9.6)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "solid"
%	 points= "(38.4,9.6);(38.4,9.6);(44.8,9.6);(44.8,9.6);(44.8,9.6);(41.6,6.4);
%	(41.6,6.4);(41.6,6.4);(38.4,9.6);(38.4,9.6);(38.4,9.6);(38.4,9.6);
%	(38.4,9.6)"
%	 />
%<parallelogram stroke-width= "0.1"
%	 p3= "(32,39.2)"
%	 p1= "(6.4,34.4)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(32,34.4)"
%	 />
%<parallelogram stroke-width= "0.1"
%	 p3= "(38.4,12.8)"
%	 p1= "(38.4,12.8)"
%	 fill-style= "none"
%	 p2= "(38.4,12.8)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(19.2,36.8)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle h$
%</text>
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(17.6,34.4);(17.6,34.4);(17.6,9.6);(17.6,9.6)"
%	 />
%<parallelogram stroke-width= "0.1"
%	 p3= "(44.8,19.2)"
%	 p1= "(25.6,14.4)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(44.8,14.4)"
%	 />
%<parallelogram stroke-width= "0.1"
%	 p3= "(44.8,16.8)"
%	 p1= "(44.8,16.8)"
%	 fill-style= "none"
%	 p2= "(44.8,16.8)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(41.6,9.6);(41.6,9.6);(41.6,14.4);(41.6,14.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(28.8,6.4);(28.8,6.4);(28.8,14.4);(28.8,14.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(28.8,19.2);(28.8,19.2);(28.8,34.4);(28.8,34.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(9.6,9.6);(9.6,9.6);(9.6,34.4);(9.6,34.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(20.8,9.6);(20.8,17.07);(21.6,24);(28.8,26.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(28.8,26.4);(33.6,28);(36.8,28.8);(37.6,34.4)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(8,12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(43.2,12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16,12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35.2,16.8)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle g$
%</text>
%<parallelogram stroke-width= "0.1"
%	 p3= "(44.8,39.2)"
%	 p1= "(35.2,34.4)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(44.8,34.4)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,36.8)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle f$
%</text>
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(35.2,6.4);(35.2,6.4);(35.2,14.4);(35.2,14.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(42.4,28);(42.4,28);(42.4,34.4);(42.4,34.4)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(43.5,32)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<multicurve stroke-width= "0.1"
%	 fill-style= "solid"
%	 points= "(39.2,29.6);(39.2,29.6);(45.6,29.6);(45.6,29.6);(45.6,29.6);(42.4,26.4);
%	(42.4,26.4);(42.4,26.4);(39.2,29.6);(39.2,29.6);(39.2,29.6);(39.2,29.6);
%	(39.2,29.6)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(12.8,39.2);(12.8,39.2);(12.8,46.4);(12.8,46.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(40,39.2);(40,39.2);(40,43.2);(40,43.2)"
%	 />
%<multicurve stroke-width= "0.1"
%	 fill-style= "none"
%	 points= "(25.6,39.2);(25.6,39.2);(25.6,46.4);(25.6,46.4)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(11.2,41.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.2,41.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(41.6,41.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle C$
%</text>
%<ellipse stroke-width= "0.1"
%	 closure= "open"
%	 p3= "(29.8,27.4)"
%	 p1= "(27.8,25.4)"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(29.8,25.4)"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.8,26.4)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle c$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.2,12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(33.6,12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.4,32)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(22.4,12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.2,20.8)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle I\otimes I\otimes D\otimes D\otimes I$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(53.4,7.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,12.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes B\otimes D\otimes D \otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65.5,19)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes B\otimes D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,25.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes D\otimes B\otimes I$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,40.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B\otimes X\otimes C$
%</text>
%<multicurve stroke-width= "0.1"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,7.2);(65,7.2);(65,10.8);(65,10.8)"
%	 />
%<multicurve stroke-width= "0.1"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,14.4);(65,14.4);(65,18);(65,18)"
%	 />
%<multicurve stroke-width= "0.1"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,20.5);(65,20.5);(65,24.5);(65,24.5)"
%	 />
%<multicurve stroke-width= "0.1"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,27);(65,27);(65,31.4);(65,31.4)"
%	 />
%<multicurve stroke-width= "0.1"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,34.5);(65,34.5);(65,38.5);(65,38.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70.5,21.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle X\otimes A\otimes c\otimes r$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(71.8,8.4)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle x\otimes a\otimes D\otimes D\otimes x$
%</text>
%<multicurve stroke-width= "0.1"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(36.8,43.2);(36.8,43.2);(40,46.4);(40,46.4);(40,46.4);(43.2,43.2);
%	(43.2,43.2);(43.2,43.2);(36.8,43.2);(36.8,43.2)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,44.4)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle b$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(19.2,8.4)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle a$
%</text>
%<multicurve stroke-width= "0.1"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,42);(65,42);(65,46);(65,46)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,47.2)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B\otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(69,43.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle B\otimes X\otimes b$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70.5,15.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle X\otimes A\otimes B\otimes g$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,33)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes D\otimes B\otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(68,29)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle {\rm id}\otimes x$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(67.5,36.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle h\otimes f$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(71.8,47.2)
\pscustom[linewidth=0.1,fillstyle=solid]{\psline(6.4,9.6)(12.8,9.6)
\psline(12.8,9.6)(9.6,6.4)
\psline(9.6,6.4)(6.4,9.6)
\psbezier(6.4,9.6)(6.4,9.6)(6.4,9.6)(6.4,9.6)
}
\newrgbcolor{userFillColour}{1 1 0.4}
\pscustom[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid]{\psline(14.4,9.6)(24,9.6)
\psline(24,9.6)(19.2,6.4)
\psline(19.2,6.4)(14.4,9.6)
\psbezier(14.4,9.6)(14.4,9.6)(14.4,9.6)(14.4,9.6)
}
\pscustom[linewidth=0.1,fillstyle=solid]{\psline(38.4,9.6)(44.8,9.6)
\psline(44.8,9.6)(41.6,6.4)
\psline(41.6,6.4)(38.4,9.6)
\psbezier(38.4,9.6)(38.4,9.6)(38.4,9.6)(38.4,9.6)
}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid](6.4,34.4)(32,34.4)(32,39.2)(6.4,39.2)
\pspolygon[linewidth=0.1](38.4,12.8)(38.4,12.8)(38.4,12.8)(38.4,12.8)
\rput(19.2,36.8){$\scriptstyle h$}
\psline[linewidth=0.1](17.6,34.4)(17.6,9.6)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid](25.6,14.4)(44.8,14.4)(44.8,19.2)(25.6,19.2)
\pspolygon[linewidth=0.1](44.8,16.8)(44.8,16.8)(44.8,16.8)(44.8,16.8)
\psline[linewidth=0.1](41.6,9.6)(41.6,14.4)
\psline[linewidth=0.1](28.8,6.4)(28.8,14.4)
\psline[linewidth=0.1](28.8,19.2)(28.8,34.4)
\psline[linewidth=0.1](9.6,9.6)(9.6,34.4)
\psbezier[linewidth=0.1](20.8,9.6)(20.8,17.07)(21.6,24)(28.8,26.4)
\psbezier[linewidth=0.1](28.8,26.4)(33.6,28)(36.8,28.8)(37.6,34.4)
\rput(8,12){$\scriptstyle X$}
\rput(43.2,12){$\scriptstyle X$}
\rput(16,12){$\scriptstyle A$}
\rput(35.2,16.8){$\scriptstyle g$}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid](35.2,34.4)(44.8,34.4)(44.8,39.2)(35.2,39.2)
\rput(40,36.8){$\scriptstyle f$}
\psline[linewidth=0.1](35.2,6.4)(35.2,14.4)
\psline[linewidth=0.1](42.4,28)(42.4,34.4)
\rput(43.5,32){$\scriptstyle X$}
\pscustom[linewidth=0.1,fillstyle=solid]{\psline(39.2,29.6)(45.6,29.6)
\psline(45.6,29.6)(42.4,26.4)
\psline(42.4,26.4)(39.2,29.6)
\psbezier(39.2,29.6)(39.2,29.6)(39.2,29.6)(39.2,29.6)
}
\psline[linewidth=0.1](12.8,39.2)(12.8,46.4)
\psline[linewidth=0.1](40,39.2)(40,43.2)
\psline[linewidth=0.1](25.6,39.2)(25.6,46.4)
\rput(11.2,41.6){$\scriptstyle B$}
\rput(27.2,41.6){$\scriptstyle X$}
\rput(41.6,41.6){$\scriptstyle C$}
\newrgbcolor{userFillColour}{1 1 0.4}
\rput{0}(28.8,26.4){\psellipse[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid](0,0)(1,1)}
\rput(28.8,26.4){$\scriptstyle c$}
\rput(27.2,12){$\scriptstyle D$}
\rput(33.6,12){$\scriptstyle D$}
\rput(38.4,32){$\scriptstyle B$}
\rput(22.4,12){$\scriptstyle B$}
\rput(27.2,20.8){$\scriptstyle D$}
\rput(65,5.6){$\scriptstyle I\otimes I\otimes D\otimes D\otimes I$}
\rput(53.4,7.6){}
\rput(65,12.5){$\scriptstyle X\otimes A\otimes B\otimes D\otimes D \otimes X$}
\rput(65.5,19){$\scriptstyle X\otimes A\otimes B\otimes D$}
\rput(65,25.5){$\scriptstyle X\otimes A\otimes D\otimes B\otimes I$}
\rput(65,40.5){$\scriptstyle B\otimes X\otimes C$}
\psline[linewidth=0.1]{->}(65,7.2)(65,10.8)
\psline[linewidth=0.1]{->}(65,14.4)(65,18)
\psline[linewidth=0.1]{->}(65,20.5)(65,24.5)
\psline[linewidth=0.1]{->}(65,27)(65,31.4)
\psline[linewidth=0.1]{->}(65,34.5)(65,38.5)
\rput(70.5,21.5){$\scriptscriptstyle X\otimes A\otimes c\otimes r$}
\rput(71.8,8.4){$\scriptscriptstyle x\otimes a\otimes D\otimes D\otimes x$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.1,fillcolor=userFillColour,fillstyle=solid](36.8,43.2)
(40,46.4)
(43.2,43.2)(36.8,43.2)
\rput(40,44.4){$\scriptstyle b$}
\rput(19.2,8.4){$\scriptstyle a$}
\psline[linewidth=0.1]{->}(65,42)(65,46)
\rput(65,47.2){$\scriptstyle B\otimes X$}
\rput(69,43.5){$\scriptscriptstyle B\otimes X\otimes b$}
\rput(70.5,15.5){$\scriptscriptstyle X\otimes A\otimes B\otimes g$}
\rput(65,33){$\scriptstyle X\otimes A\otimes D\otimes B\otimes X$}
\rput(68,29){$\scriptscriptstyle {\rm id}\otimes x$}
\rput(67.5,36.5){$\scriptscriptstyle h\otimes f$}
\end{pspicture}


==> PIC/geometry-2.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Fri Jan 02 16:25:11 PST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="8" x-max="87.5" y-min="7" y-max="59" auto-bounding="true">
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 points= "(8,12);(8,12);(16,12);(16,12);(16,12);(12,8);
%	(12,8);(12,8);(8,12);(8,12);(8,12);(8,12);
%	(8,12)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(18,12);(18,12);(30,12);(30,12);(30,12);(24,8);
%	(24,8);(24,8);(18,12);(18,12);(18,12);(18,12);
%	(18,12)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 points= "(48,12);(48,12);(56,12);(56,12);(56,12);(52,8);
%	(52,8);(52,8);(48,12);(48,12);(48,12);(48,12);
%	(48,12)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(40,49)"
%	 p1= "(8,43)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(40,43)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(48,16)"
%	 p1= "(48,16)"
%	 fill-style= "none"
%	 p2= "(48,16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,46)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle h$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(22,43);(22,43);(22,12);(22,12)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(56,24)"
%	 p1= "(32,18)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(56,18)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(56,21)"
%	 p1= "(56,21)"
%	 fill-style= "none"
%	 p2= "(56,21)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(52,12);(52,12);(52,18);(52,18)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(36,8);(36,8);(36,18);(36,18)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(36,24);(36,24);(36,43);(36,43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(12,12);(12,12);(12,43);(12,43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(26,12);(26,21.34);(27,30);(36,33)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(36,33);(42,35);(46,36);(47,43)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,21)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle g$
%</text>
%<parallelogram stroke-width= "0.12"
%	 p3= "(56,49)"
%	 p1= "(44,43)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(56,43)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,46)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle f$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(44,8);(44,8);(44,18);(44,18)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(53,35);(53,35);(53,43);(53,43)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 points= "(49,37);(49,37);(57,37);(57,37);(57,37);(53,33);
%	(53,33);(53,33);(49,37);(49,37);(49,37);(49,37);
%	(49,37)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(16,49);(16,49);(16,58);(16,58)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(50,49);(50,49);(50,54);(50,54)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(32,49);(32,49);(32,58);(32,58)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(14,52)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,52)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52,52)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle C$
%</text>
%<ellipse stroke-width= "0.12"
%	 closure= "open"
%	 p3= "(37.25,34.25)"
%	 p1= "(34.75,31.75)"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(37.25,31.75)"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(36,33)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle c$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(48,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(28,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,26)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,7)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle I\otimes I\otimes D\otimes D\otimes I$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(64.5,9.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,15.63)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes B\otimes D\otimes D \otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79.63,23.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes B\otimes D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,31.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes D\otimes B\otimes I$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,50.63)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B\otimes X\otimes C$
%</text>
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(79,9);(79,9);(79,13.5);(79,13.5)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(79,18);(79,18);(79,22.5);(79,22.5)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(79,25.62);(79,25.62);(79,30.63);(79,30.63)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(79,33.75);(79,33.75);(79,39.25);(79,39.25)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(79,43.13);(79,43.13);(79,48.13);(79,48.13)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(85.88,26.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle X\otimes A\otimes c\otimes r$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,10.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle x\otimes a\otimes D\otimes D\otimes x$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(46,54);(46,54);(50,58);(50,58);(50,58);(54,54);
%	(54,54);(54,54);(46,54);(46,54)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,55.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle b$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,10.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle a$
%</text>
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(79,52.5);(79,52.5);(79,57.5);(79,57.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,59)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B\otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(84,54.38)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle B\otimes X\otimes b$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85.88,19.38)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle X\otimes A\otimes B\otimes g$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,41.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes D\otimes B\otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.75,36.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle {\rm id}\otimes x$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.13,45.63)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle h\otimes f$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(87.5,59)
\pscustom[linewidth=0.12,fillstyle=solid]{\psline(8,12)(16,12)
\psline(16,12)(12,8)
\psline(12,8)(8,12)
\psbezier(8,12)(8,12)(8,12)(8,12)
}
\newrgbcolor{userFillColour}{1 1 0.4}
\pscustom[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid]{\psline(18,12)(30,12)
\psline(30,12)(24,8)
\psline(24,8)(18,12)
\psbezier(18,12)(18,12)(18,12)(18,12)
}
\pscustom[linewidth=0.12,fillstyle=solid]{\psline(48,12)(56,12)
\psline(56,12)(52,8)
\psline(52,8)(48,12)
\psbezier(48,12)(48,12)(48,12)(48,12)
}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](8,43)(40,43)(40,49)(8,49)
\pspolygon[linewidth=0.12](48,16)(48,16)(48,16)(48,16)
\rput(24,46){$\scriptstyle h$}
\psline[linewidth=0.12](22,43)(22,12)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](32,18)(56,18)(56,24)(32,24)
\pspolygon[linewidth=0.12](56,21)(56,21)(56,21)(56,21)
\psline[linewidth=0.12](52,12)(52,18)
\psline[linewidth=0.12](36,8)(36,18)
\psline[linewidth=0.12](36,24)(36,43)
\psline[linewidth=0.12](12,12)(12,43)
\psbezier[linewidth=0.12](26,12)(26,21.34)(27,30)(36,33)
\psbezier[linewidth=0.12](36,33)(42,35)(46,36)(47,43)
\rput(10,15){$\scriptstyle X$}
\rput(54,15){$\scriptstyle X$}
\rput(20,15){$\scriptstyle A$}
\rput(44,21){$\scriptstyle g$}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](44,43)(56,43)(56,49)(44,49)
\rput(50,46){$\scriptstyle f$}
\psline[linewidth=0.12](44,8)(44,18)
\psline[linewidth=0.12](53,35)(53,43)
\rput(54.38,40){$\scriptstyle X$}
\pscustom[linewidth=0.12,fillstyle=solid]{\psline(49,37)(57,37)
\psline(57,37)(53,33)
\psline(53,33)(49,37)
\psbezier(49,37)(49,37)(49,37)(49,37)
}
\psline[linewidth=0.12](16,49)(16,58)
\psline[linewidth=0.12](50,49)(50,54)
\psline[linewidth=0.12](32,49)(32,58)
\rput(14,52){$\scriptstyle B$}
\rput(34,52){$\scriptstyle X$}
\rput(52,52){$\scriptstyle C$}
\newrgbcolor{userFillColour}{1 1 0.4}
\rput{0}(36,33){\psellipse[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](0,0)(1.25,1.25)}
\rput(36,33){$\scriptstyle c$}
\rput(34,15){$\scriptstyle D$}
\rput(42,15){$\scriptstyle D$}
\rput(48,40){$\scriptstyle B$}
\rput(28,15){$\scriptstyle B$}
\rput(34,26){$\scriptstyle D$}
\rput(79,7){$\scriptstyle I\otimes I\otimes D\otimes D\otimes I$}
\rput(64.5,9.5){}
\rput(79,15.63){$\scriptstyle X\otimes A\otimes B\otimes D\otimes D \otimes X$}
\rput(79.63,23.75){$\scriptstyle X\otimes A\otimes B\otimes D$}
\rput(79,31.88){$\scriptstyle X\otimes A\otimes D\otimes B\otimes I$}
\rput(79,50.63){$\scriptstyle B\otimes X\otimes C$}
\psline[linewidth=0.12]{->}(79,9)(79,13.5)
\psline[linewidth=0.12]{->}(79,18)(79,22.5)
\psline[linewidth=0.12]{->}(79,25.62)(79,30.63)
\psline[linewidth=0.12]{->}(79,33.75)(79,39.25)
\psline[linewidth=0.12]{->}(79,43.13)(79,48.13)
\rput(85.88,26.88){$\scriptscriptstyle X\otimes A\otimes c\otimes r$}
\rput(87.5,10.5){$\scriptscriptstyle x\otimes a\otimes D\otimes D\otimes x$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](46,54)
(50,58)
(54,54)(46,54)
\rput(50,55.5){$\scriptstyle b$}
\rput(24,10.5){$\scriptstyle a$}
\psline[linewidth=0.12]{->}(79,52.5)(79,57.5)
\rput(79,59){$\scriptstyle B\otimes X$}
\rput(84,54.38){$\scriptscriptstyle B\otimes X\otimes b$}
\rput(85.88,19.38){$\scriptscriptstyle X\otimes A\otimes B\otimes g$}
\rput(79,41.25){$\scriptstyle X\otimes A\otimes D\otimes B\otimes X$}
\rput(82.75,36.25){$\scriptscriptstyle {\rm id}\otimes x$}
\rput(82.13,45.63){$\scriptscriptstyle h\otimes f$}
\end{pspicture}


==> PIC/geometry-3.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Fri Jan 02 17:07:59 PST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="8" x-max="93.5" y-min="7" y-max="59" auto-bounding="true">
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 points= "(8,12);(8,12);(16,12);(16,12);(16,12);(12,8);
%	(12,8);(12,8);(8,12);(8,12);(8,12);(8,12);
%	(8,12)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(18,12);(18,12);(30,12);(30,12);(30,12);(24,8);
%	(24,8);(24,8);(18,12);(18,12);(18,12);(18,12);
%	(18,12)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 points= "(48,12);(48,12);(56,12);(56,12);(56,12);(52,8);
%	(52,8);(52,8);(48,12);(48,12);(48,12);(48,12);
%	(48,12)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(40,49)"
%	 p1= "(8,43)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(40,43)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(48,16)"
%	 p1= "(48,16)"
%	 fill-style= "none"
%	 p2= "(48,16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,46)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle h$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(22,43);(22,43);(22,12);(22,12)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(56,24)"
%	 p1= "(32,18)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(56,18)"
%	 />
%<parallelogram stroke-width= "0.12"
%	 p3= "(56,21)"
%	 p1= "(56,21)"
%	 fill-style= "none"
%	 p2= "(56,21)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(52,12);(52,12);(52,18);(52,18)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(36,8);(36,8);(36,18);(36,18)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(36,24);(36,24);(36,43);(36,43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(12,12);(12,12);(12,43);(12,43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(26,12);(26,21.34);(27,30);(36,33)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(36,33);(42,35);(46,36);(47,43)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,21)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle g$
%</text>
%<parallelogram stroke-width= "0.12"
%	 p3= "(56,49)"
%	 p1= "(44,43)"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(56,43)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,46)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle f$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(44,8);(44,8);(44,18);(44,18)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(53,35);(53,35);(53,43);(53,43)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 points= "(49,37);(49,37);(57,37);(57,37);(57,37);(53,33);
%	(53,33);(53,33);(49,37);(49,37);(49,37);(49,37);
%	(49,37)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(16,49);(16,49);(16,58);(16,58)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(50,49);(50,49);(50,54);(50,54)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(32,49);(32,49);(32,58);(32,58)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(14,52)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,52)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52,52)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle C$
%</text>
%<ellipse stroke-width= "0.12"
%	 closure= "open"
%	 p3= "(37.25,34.25)"
%	 p1= "(34.75,31.75)"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 p2= "(37.25,31.75)"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(36,33)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle c$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(48,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(28,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,26)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,7)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle I\otimes I\otimes D\otimes D\otimes I$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70.5,9.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,15.63)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes B\otimes D\otimes D \otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85.63,23.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes B\otimes D$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,31.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes D\otimes B\otimes I$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,50.63)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B\otimes X\otimes C$
%</text>
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(85,9);(85,9);(85,13.5);(85,13.5)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(85,18);(85,18);(85,22.5);(85,22.5)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(85,25.62);(85,25.62);(85,30.63);(85,30.63)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(85,33.75);(85,33.75);(85,39.25);(85,39.25)"
%	 />
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(85,43.13);(85,43.13);(85,48.13);(85,48.13)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(91.88,26.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle X\otimes A\otimes c\otimes r$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(93.5,10.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle x\otimes a\otimes D\otimes D\otimes x$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(46,54);(46,54);(50,58);(50,58);(50,58);(54,54);
%	(54,54);(54,54);(46,54);(46,54)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,55.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle b$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,10.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle a$
%</text>
%<multicurve stroke-width= "0.12"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(85,52.5);(85,52.5);(85,57.5);(85,57.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,59)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle B\otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,54.38)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle B\otimes X\otimes b$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(91.88,19.38)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle X\otimes A\otimes B\otimes g$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,41.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptstyle X\otimes A\otimes D\otimes B\otimes X$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(88.75,36.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle {\rm id}\otimes x$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(88.13,45.63)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\scriptscriptstyle h\otimes f$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(93.5,59)
\pscustom[linewidth=0.12,fillstyle=solid]{\psline(8,12)(16,12)
\psline(16,12)(12,8)
\psline(12,8)(8,12)
\psbezier(8,12)(8,12)(8,12)(8,12)
}
\newrgbcolor{userFillColour}{1 1 0.4}
\pscustom[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid]{\psline(18,12)(30,12)
\psline(30,12)(24,8)
\psline(24,8)(18,12)
\psbezier(18,12)(18,12)(18,12)(18,12)
}
\pscustom[linewidth=0.12,fillstyle=solid]{\psline(48,12)(56,12)
\psline(56,12)(52,8)
\psline(52,8)(48,12)
\psbezier(48,12)(48,12)(48,12)(48,12)
}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](8,43)(40,43)(40,49)(8,49)
\pspolygon[linewidth=0.12](48,16)(48,16)(48,16)(48,16)
\rput(24,46){$\scriptstyle h$}
\psline[linewidth=0.12](22,43)(22,12)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](32,18)(56,18)(56,24)(32,24)
\pspolygon[linewidth=0.12](56,21)(56,21)(56,21)(56,21)
\psline[linewidth=0.12](52,12)(52,18)
\psline[linewidth=0.12](36,8)(36,18)
\psline[linewidth=0.12](36,24)(36,43)
\psline[linewidth=0.12](12,12)(12,43)
\psbezier[linewidth=0.12](26,12)(26,21.34)(27,30)(36,33)
\psbezier[linewidth=0.12](36,33)(42,35)(46,36)(47,43)
\rput(10,15){$\scriptstyle X$}
\rput(54,15){$\scriptstyle X$}
\rput(20,15){$\scriptstyle A$}
\rput(44,21){$\scriptstyle g$}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](44,43)(56,43)(56,49)(44,49)
\rput(50,46){$\scriptstyle f$}
\psline[linewidth=0.12](44,8)(44,18)
\psline[linewidth=0.12](53,35)(53,43)
\rput(54.38,40){$\scriptstyle X$}
\pscustom[linewidth=0.12,fillstyle=solid]{\psline(49,37)(57,37)
\psline(57,37)(53,33)
\psline(53,33)(49,37)
\psbezier(49,37)(49,37)(49,37)(49,37)
}
\psline[linewidth=0.12](16,49)(16,58)
\psline[linewidth=0.12](50,49)(50,54)
\psline[linewidth=0.12](32,49)(32,58)
\rput(14,52){$\scriptstyle B$}
\rput(34,52){$\scriptstyle X$}
\rput(52,52){$\scriptstyle C$}
\newrgbcolor{userFillColour}{1 1 0.4}
\rput{0}(36,33){\psellipse[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](0,0)(1.25,1.25)}
\rput(36,33){$\scriptstyle c$}
\rput(34,15){$\scriptstyle D$}
\rput(42,15){$\scriptstyle D$}
\rput(48,40){$\scriptstyle B$}
\rput(28,15){$\scriptstyle B$}
\rput(34,26){$\scriptstyle D$}
\rput(85,7){$\scriptstyle I\otimes I\otimes D\otimes D\otimes I$}
\rput(70.5,9.5){}
\rput(85,15.63){$\scriptstyle X\otimes A\otimes B\otimes D\otimes D \otimes X$}
\rput(85.63,23.75){$\scriptstyle X\otimes A\otimes B\otimes D$}
\rput(85,31.88){$\scriptstyle X\otimes A\otimes D\otimes B\otimes I$}
\rput(85,50.63){$\scriptstyle B\otimes X\otimes C$}
\psline[linewidth=0.12]{->}(85,9)(85,13.5)
\psline[linewidth=0.12]{->}(85,18)(85,22.5)
\psline[linewidth=0.12]{->}(85,25.62)(85,30.63)
\psline[linewidth=0.12]{->}(85,33.75)(85,39.25)
\psline[linewidth=0.12]{->}(85,43.13)(85,48.13)
\rput(91.88,26.88){$\scriptscriptstyle X\otimes A\otimes c\otimes r$}
\rput(93.5,10.5){$\scriptscriptstyle x\otimes a\otimes D\otimes D\otimes x$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.12,fillcolor=userFillColour,fillstyle=solid](46,54)
(50,58)
(54,54)(46,54)
\rput(50,55.5){$\scriptstyle b$}
\rput(24,10.5){$\scriptstyle a$}
\psline[linewidth=0.12]{->}(85,52.5)(85,57.5)
\rput(85,59){$\scriptstyle B\otimes X$}
\rput(90,54.38){$\scriptscriptstyle B\otimes X\otimes b$}
\rput(91.88,19.38){$\scriptscriptstyle X\otimes A\otimes B\otimes g$}
\rput(85,41.25){$\scriptstyle X\otimes A\otimes D\otimes B\otimes X$}
\rput(88.75,36.25){$\scriptscriptstyle {\rm id}\otimes x$}
\rput(88.13,45.63){$\scriptscriptstyle h\otimes f$}
\end{pspicture}


==> PIC/geometry.tex <==
%Created by jPicEdt 1.x
%PsTricks format (pstricks.sty needed)
%Fri Aug 03 16:37:58 BST 2007
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\begin{pspicture}(0,0)(93.50,59.00)
\psline[linewidth=0.12,linecolor=black,fillcolor=black,fillstyle=solid]{-}(8.00,12.00)(16.00,12.00)(12.00,8.00)(8.00,12.00)(8.00,12.00)
\newrgbcolor{userFillColour}{1.00 1.00 0.40}
\psline[linewidth=0.12,linecolor=black,fillcolor=userFillColour,fillstyle=solid]{-}(18.00,12.00)(30.00,12.00)(24.00,8.00)(18.00,12.00)(18.00,12.00)
\psline[linewidth=0.12,linecolor=black,fillcolor=black,fillstyle=solid]{-}(48.00,12.00)(56.00,12.00)(52.00,8.00)(48.00,12.00)(48.00,12.00)
\newrgbcolor{userFillColour}{1.00 1.00 0.40}
\psframe[linewidth=0.12,linecolor=black,fillcolor=userFillColour,fillstyle=solid](8.00,43.00)(40.00,49.00)
\psframe[linewidth=0.12,linecolor=black](48.00,16.00)(48.00,16.00)
\rput(24.00,46.00){$\scriptstyle h$}
\psline[linewidth=0.12,linecolor=black]{-}(22.00,43.00)(22.00,12.00)
\newrgbcolor{userFillColour}{1.00 1.00 0.40}
\psframe[linewidth=0.12,linecolor=black,fillcolor=userFillColour,fillstyle=solid](32.00,18.00)(56.00,24.00)
\psframe[linewidth=0.12,linecolor=black](56.00,21.00)(56.00,21.00)
\psline[linewidth=0.12,linecolor=black]{-}(52.00,12.00)(52.00,18.00)
\psline[linewidth=0.12,linecolor=black]{-}(36.00,8.00)(36.00,18.00)
\psline[linewidth=0.12,linecolor=black]{-}(36.00,24.00)(36.00,43.00)
\psline[linewidth=0.12,linecolor=black]{-}(12.00,12.00)(12.00,43.00)
\psbezier[linewidth=0.12,linecolor=black]{-}(26.00,12.00)(26.00,21.34)(27.00,30.00)(36.00,33.00)
\psbezier[linewidth=0.12,linecolor=black]{-}(36.00,33.00)(42.00,35.00)(46.00,36.00)(47.00,43.00)
\rput(10.00,15.00){$\scriptstyle X$}
\rput(54.00,15.00){$\scriptstyle X$}
\rput(20.00,15.00){$\scriptstyle A$}
\rput(44.00,21.00){$\scriptstyle g$}
\newrgbcolor{userFillColour}{1.00 1.00 0.40}
\psframe[linewidth=0.12,linecolor=black,fillcolor=userFillColour,fillstyle=solid](44.00,43.00)(56.00,49.00)
\rput(50.00,46.00){$\scriptstyle f$}
\psline[linewidth=0.12,linecolor=black]{-}(44.00,8.00)(44.00,18.00)
\psline[linewidth=0.12,linecolor=black]{-}(53.00,35.00)(53.00,43.00)
\rput(54.38,40.00){$\scriptstyle X$}
\psline[linewidth=0.12,linecolor=black,fillcolor=black,fillstyle=solid]{-}(49.00,37.00)(57.00,37.00)(53.00,33.00)(49.00,37.00)(49.00,37.00)
\psline[linewidth=0.12,linecolor=black]{-}(16.00,49.00)(16.00,58.00)
\psline[linewidth=0.12,linecolor=black]{-}(50.00,49.00)(50.00,54.00)
\psline[linewidth=0.12,linecolor=black]{-}(32.00,49.00)(32.00,58.00)
\rput(14.00,52.00){$\scriptstyle B$}
\rput(34.00,52.00){$\scriptstyle X$}
\rput(52.00,52.00){$\scriptstyle C$}
\newrgbcolor{userFillColour}{1.00 1.00 0.40}
\pscircle[linewidth=0.12,linecolor=black,fillcolor=userFillColour,fillstyle=solid](36.00,33.00){1.25}
\rput(36.00,33.00){$\scriptstyle c$}
\rput(34.00,15.00){$\scriptstyle D$}
\rput(42.00,15.00){$\scriptstyle D$}
\rput(48.00,40.00){$\scriptstyle B$}
\rput(28.00,15.00){$\scriptstyle B$}
\rput(34.00,26.00){$\scriptstyle D$}
\rput(85.00,7.00){$\scriptstyle I\otimes I\otimes D\otimes D\otimes I$}
\rput(70.50,9.50){}
\rput(85.00,15.63){$\scriptstyle X\otimes A\otimes B\otimes D\otimes D \otimes X$}
\rput(85.63,23.75){$\scriptstyle X\otimes A\otimes B\otimes D$}
\rput(85.00,31.88){$\scriptstyle X\otimes A\otimes D\otimes B\otimes I$}
\rput(85.00,50.63){$\scriptstyle B\otimes X\otimes C$}
\psline[linewidth=0.12,linecolor=black]{->}(85.00,9.00)(85.00,13.50)
\psline[linewidth=0.12,linecolor=black]{->}(85.00,18.00)(85.00,22.50)
\psline[linewidth=0.12,linecolor=black]{->}(85.00,25.62)(85.00,30.63)
\psline[linewidth=0.12,linecolor=black]{->}(85.00,33.75)(85.00,39.25)
\psline[linewidth=0.12,linecolor=black]{->}(85.00,43.13)(85.00,48.13)
\rput(91.88,26.88){$\scriptscriptstyle X\otimes A\otimes c\otimes r$}
\rput(93.50,10.50){$\scriptscriptstyle x\otimes a\otimes D\otimes D\otimes x$}
\newrgbcolor{userFillColour}{1.00 1.00 0.40}
\psline[linewidth=0.12,linecolor=black,fillcolor=userFillColour,fillstyle=solid]{-}(46.00,54.00)(50.00,58.00)(54.00,54.00)(46.00,54.00)
\rput(50.00,55.50){$\scriptstyle b$}
\rput(24.00,10.50){$\scriptstyle a$}
\psline[linewidth=0.12,linecolor=black]{->}(85.00,52.50)(85.00,57.50)
\rput(85.00,59.00){$\scriptstyle B\otimes X$}
\rput(90.00,54.38){$\scriptscriptstyle B\otimes X\otimes b$}
\rput(91.88,19.38){$\scriptscriptstyle X\otimes A\otimes B\otimes g$}
\rput(85.00,41.25){$\scriptstyle X\otimes A\otimes D\otimes B\otimes X$}
\rput(88.75,36.25){$\scriptscriptstyle {\rm id}\otimes x$}
\rput(88.13,45.63){$\scriptscriptstyle h\otimes f$}
\end{pspicture}


==> PIC/nab.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 18 00:17:23 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="92" y-min="-1.66" y-max="55" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,41.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(81.25,38.25);(81.25,38.25);(81.25,51.25);(81.25,51.25)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(70.62,51.37);(70.62,51.37);(70.62,46.75);(70.62,46.75)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(66.88,30.75);(66.88,30.75);(66.88,43.12);(66.88,43.12)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(78.17,37.49);(78.17,37.49);(78.12,30.75);(78.12,30.75)"
%	 />
%<multicurve stroke-width= "0.22"
%	 right-arrow= "head"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(76.62,42.75);(76.62,42.75);(64.62,42.75);(64.62,42.75);(64.62,42.75);(67.62,46.75);
%	(67.62,46.75);(67.62,46.75);(73.62,46.75);(73.62,46.75);(73.62,46.75);(76.62,42.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70.62,44.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monoid$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(74.38,38.12);(74.38,38.12);(74.38,42.63);(74.38,42.63)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(70.05,33.59);(70.05,33.59);(67.04,29.59);(67.04,29.59);(67.04,29.59);(64.04,33.59);
%	(64.04,33.59);(64.04,33.59);(70.05,33.59);(70.05,33.59)"
%	 />
%<multicurve stroke-width= "0.22"
%	 right-arrow= "head"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(72,40.5);(72,40.5);(84,40.5);(84,40.5);(84,40.5);(81,36.5);
%	(81,36.5);(81,36.5);(75,36.5);(75,36.5);(75,36.5);(72,40.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(78,38.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonoid$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(36.25,46.88);(36.25,46.88);(36.25,54.12);(36.25,54.12)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(45,52.25);(45,52.25);(45,46.62);(45,46.62)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(40.62,39.13);(40.62,39.13);(40.62,45.62);(40.62,45.62)"
%	 />
%<multicurve stroke-width= "0.22"
%	 right-arrow= "head"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(34.62,47);(34.62,47);(46.62,47);(46.62,47);(46.62,47);(43.62,43);
%	(43.62,43);(43.62,43);(37.62,43);(37.62,43);(37.62,43);(34.62,47)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(36.25,37.25);(36.25,37.25);(36.25,31.52);(36.25,31.52)"
%	 />
%<multicurve stroke-width= "0.22"
%	 right-arrow= "head"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(47,37.25);(47,37.25);(35,37.25);(35,37.25);(35,37.25);(38,41.25);
%	(38,41.25);(38,41.25);(44,41.25);(44,41.25);(44,41.25);(47,37.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40.62,39.13)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monoid$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(44.38,29.75);(44.38,29.75);(44.38,37.25);(44.38,37.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40.62,45)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonoid$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(41.92,50.7);(41.92,50.7);(44.92,54.7);(44.92,54.7);(44.92,54.7);(47.92,50.7);
%	(47.92,50.7);(47.92,50.7);(41.92,50.7);(41.92,50.7)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(39.2,33.95);(39.2,33.95);(36.2,29.95);(36.2,29.95);(36.2,29.95);(33.2,33.95);
%	(33.2,33.95);(33.2,33.95);(39.2,33.95);(39.2,33.95)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(33.75,31.63)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(46.88,54.75)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<multicurve stroke-width= "0.22"
%	 right-arrow= "head"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(3.38,46.62);(3.38,46.62);(15.38,46.62);(15.38,46.62);(15.38,46.62);(12.38,42.62);
%	(12.38,42.62);(12.38,42.62);(6.38,42.62);(6.38,42.62);(6.38,42.62);(3.38,46.62)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(9.38,42.62);(9.38,42.62);(9.38,38.64);(9.38,38.64)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,44.62)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonoid$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(12.32,41.08);(12.32,41.08);(9.32,37.08);(9.32,37.08);(9.32,37.08);(6.32,41.08);
%	(6.32,41.08);(6.32,41.08);(12.32,41.08);(12.32,41.08)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(6.88,38.75)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(33.12,50.62);(33.12,50.62);(36.12,54.62);(36.12,54.62);(36.12,54.62);(39.12,50.62);
%	(39.12,50.62);(39.12,50.62);(33.12,50.62);(33.12,50.62)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(5,46.88);(5,46.88);(5,54.12);(5,54.12)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(13.75,52.25);(13.75,52.25);(13.75,46.62);(13.75,46.62)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(10.67,50.7);(10.67,50.7);(13.67,54.7);(13.67,54.7);(13.67,54.7);(16.67,50.7);
%	(16.67,50.7);(16.67,50.7);(10.67,50.7);(10.67,50.7)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.63,54.75)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(1.88,50.62);(1.88,50.62);(4.88,54.62);(4.88,54.62);(4.88,54.62);(7.88,50.62);
%	(7.88,50.62);(7.88,50.62);(1.88,50.62);(1.88,50.62)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(47.5,33.75);(47.5,33.75);(44.5,29.75);(44.5,29.75);(44.5,29.75);(41.5,33.75);
%	(41.5,33.75);(41.5,33.75);(47.5,33.75);(47.5,33.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,41.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(81.25,33.75);(81.25,33.75);(78.25,29.75);(78.25,29.75);(78.25,29.75);(75.25,33.75);
%	(75.25,33.75);(75.25,33.75);(81.25,33.75);(81.25,33.75)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(78.38,50.62);(78.38,50.62);(81.38,54.62);(81.38,54.62);(81.38,54.62);(84.38,50.62);
%	(84.38,50.62);(84.38,50.62);(78.38,50.62);(78.38,50.62)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(67.5,50.62);(67.5,50.62);(70.5,54.62);(70.5,54.62);(70.5,54.62);(73.5,50.62);
%	(73.5,50.62);(73.5,50.62);(67.5,50.62);(67.5,50.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(92,41.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(83.75,54.38)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(68.12,54.38)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34.38,55)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,54.38)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(45,7);(45,7);(45,20);(45,20)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(30,-0.5);(30,-0.5);(30,16.88);(30,16.88)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(41.3,6.24);(41.3,6.24);(41.25,-0.5);(41.25,-0.5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(37.5,6.88);(37.5,6.88);(37.5,16.25);(37.5,16.25)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(33.17,2.34);(33.17,2.34);(30.17,-1.66);(30.17,-1.66);(30.17,-1.66);(27.17,2.34);
%	(27.17,2.34);(27.17,2.34);(33.17,2.34);(33.17,2.34)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(64.38,31.25)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<multicurve stroke-width= "0.22"
%	 right-arrow= "head"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(35.12,9.25);(35.12,9.25);(47.12,9.25);(47.12,9.25);(47.12,9.25);(44.12,5.25);
%	(44.12,5.25);(44.12,5.25);(38.12,5.25);(38.12,5.25);(38.12,5.25);(35.12,9.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(41.12,7.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonoid$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(44.38,2.5);(44.38,2.5);(41.37,-1.5);(41.37,-1.5);(41.37,-1.5);(38.37,2.5);
%	(38.37,2.5);(38.37,2.5);(44.38,2.5);(44.38,2.5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(42,16);(42,16);(45,20);(45,20);(45,20);(48,16);
%	(48,16);(48,16);(42,16);(42,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(27,16);(27,16);(30,20);(30,20);(30,20);(33,16);
%	(33,16);(33,16);(27,16);(27,16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55.12,10.62)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,19.38)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.12,19.38)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(34.5,16);(34.5,16);(37.5,20);(37.5,20);(37.5,20);(40.5,16);
%	(40.5,16);(40.5,16);(34.5,16);(34.5,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(67.5,-0.5);(67.5,-0.5);(67.5,16.88);(67.5,16.88)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(78.75,16.88);(78.75,16.88);(78.74,-0.5);(78.74,-0.5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(70.67,2.34);(70.67,2.34);(67.67,-1.66);(67.67,-1.66);(67.67,-1.66);(64.67,2.34);
%	(64.67,2.34);(64.67,2.34);(70.67,2.34);(70.67,2.34)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,-0.62)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 fill-color= "#ffff66"
%	 points= "(81.88,2.5);(81.88,2.5);(78.87,-1.5);(78.87,-1.5);(78.87,-1.5);(75.87,2.5);
%	(75.87,2.5);(75.87,2.5);(81.88,2.5);(81.88,2.5)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(75.75,16);(75.75,16);(78.75,20);(78.75,20);(78.75,20);(81.75,16);
%	(81.75,16);(81.75,16);(75.75,16);(75.75,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "solid"
%	 points= "(64.5,16);(64.5,16);(67.5,20);(67.5,20);(67.5,20);(70.5,16);
%	(70.5,16);(70.5,16);(64.5,16);(64.5,16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.25,19.38)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65.62,19.38)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.5,0)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,31.25)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80.62,31.25)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.25,0)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,0)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\monunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(39.38,19.38)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\comonunit$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,10.62)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(92,55)
\rput(25,41.88){$\eqls$}
\psline[linewidth=0.22](81.25,38.25)(81.25,51.25)
\psline[linewidth=0.22](70.62,51.37)(70.62,46.75)
\psline[linewidth=0.22](66.88,30.75)(66.88,43.12)
\psline[linewidth=0.22](78.17,37.49)(78.12,30.75)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](76.62,42.75)
(64.62,42.75)
(67.62,46.75)
(73.62,46.75)(76.62,42.75)
\rput(70.62,44.75){$\monoid$}
\psline[linewidth=0.22](74.38,38.12)(74.38,42.63)
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](70.05,33.59)
(67.04,29.59)
(64.04,33.59)(70.05,33.59)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](72,40.5)
(84,40.5)
(81,36.5)
(75,36.5)(72,40.5)
\rput(78,38.5){$\comonoid$}
\psline[linewidth=0.22](36.25,46.88)(36.25,54.12)
\psline[linewidth=0.22](45,52.25)(45,46.62)
\psline[linewidth=0.22](40.62,39.13)(40.62,45.62)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](34.62,47)
(46.62,47)
(43.62,43)
(37.62,43)(34.62,47)
\psline[linewidth=0.22](36.25,37.25)(36.25,31.52)
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](47,37.25)
(35,37.25)
(38,41.25)
(44,41.25)(47,37.25)
\rput(40.62,39.13){$\monoid$}
\psline[linewidth=0.22](44.38,29.75)(44.38,37.25)
\rput(40.62,45){$\comonoid$}
\psline[linewidth=0.22,fillstyle=solid](41.92,50.7)
(44.92,54.7)
(47.92,50.7)(41.92,50.7)
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](39.2,33.95)
(36.2,29.95)
(33.2,33.95)(39.2,33.95)
\rput[r](33.75,31.63){$\monunit$}
\rput[l](46.88,54.75){$\comonunit$}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](3.38,46.62)
(15.38,46.62)
(12.38,42.62)
(6.38,42.62)(3.38,46.62)
\psline[linewidth=0.22](9.38,42.62)(9.38,38.64)
\rput(9.38,44.62){$\comonoid$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](12.32,41.08)
(9.32,37.08)
(6.32,41.08)(12.32,41.08)
\rput[r](6.88,38.75){$\monunit$}
\psline[linewidth=0.22,fillstyle=solid](33.12,50.62)
(36.12,54.62)
(39.12,50.62)(33.12,50.62)
\psline[linewidth=0.22](5,46.88)(5,54.12)
\psline[linewidth=0.22](13.75,52.25)(13.75,46.62)
\psline[linewidth=0.22,fillstyle=solid](10.67,50.7)
(13.67,54.7)
(16.67,50.7)(10.67,50.7)
\rput[l](15.63,54.75){$\comonunit$}
\psline[linewidth=0.22,fillstyle=solid](1.88,50.62)
(4.88,54.62)
(7.88,50.62)(1.88,50.62)
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](47.5,33.75)
(44.5,29.75)
(41.5,33.75)(47.5,33.75)
\rput(55,41.88){$\eqls$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](81.25,33.75)
(78.25,29.75)
(75.25,33.75)(81.25,33.75)
\psline[linewidth=0.22,fillstyle=solid](78.38,50.62)
(81.38,54.62)
(84.38,50.62)(78.38,50.62)
\psline[linewidth=0.22,fillstyle=solid](67.5,50.62)
(70.5,54.62)
(73.5,50.62)(67.5,50.62)
\rput(92,41.88){$\eqls$}
\rput[l](83.75,54.38){$\comonunit$}
\rput[r](68.12,54.38){$\comonunit$}
\rput[r](34.38,55){$\comonunit$}
\rput[r](3.12,54.38){$\comonunit$}
\psline[linewidth=0.22](45,7)(45,20)
\psline[linewidth=0.22](30,-0.5)(30,16.88)
\psline[linewidth=0.22](41.3,6.24)(41.25,-0.5)
\psline[linewidth=0.22](37.5,6.88)(37.5,16.25)
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](33.17,2.34)
(30.17,-1.66)
(27.17,2.34)(33.17,2.34)
\rput[r](64.38,31.25){$\monunit$}
\newrgbcolor{userFillColour}{1 1 0.4}
\pspolygon[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](35.12,9.25)
(47.12,9.25)
(44.12,5.25)
(38.12,5.25)(35.12,9.25)
\rput(41.12,7.25){$\comonoid$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](44.38,2.5)
(41.37,-1.5)
(38.37,2.5)(44.38,2.5)
\psline[linewidth=0.22,fillstyle=solid](42,16)
(45,20)
(48,16)(42,16)
\psline[linewidth=0.22,fillstyle=solid](27,16)
(30,20)
(33,16)(27,16)
\rput(55.12,10.62){$\eqls$}
\rput[l](47.5,19.38){$\comonunit$}
\rput[r](28.12,19.38){$\comonunit$}
\psline[linewidth=0.22,fillstyle=solid](34.5,16)
(37.5,20)
(40.5,16)(34.5,16)
\psline[linewidth=0.22](67.5,-0.5)(67.5,16.88)
\psline[linewidth=0.22](78.75,16.88)(78.74,-0.5)
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](70.67,2.34)
(67.67,-1.66)
(64.67,2.34)(70.67,2.34)
\rput[r](65,-0.62){$\monunit$}
\newrgbcolor{userFillColour}{1 1 0.4}
\psline[linewidth=0.22,fillcolor=userFillColour,fillstyle=solid](81.88,2.5)
(78.87,-1.5)
(75.87,2.5)(81.88,2.5)
\psline[linewidth=0.22,fillstyle=solid](75.75,16)
(78.75,20)
(81.75,16)(75.75,16)
\psline[linewidth=0.22,fillstyle=solid](64.5,16)
(67.5,20)
(70.5,16)(64.5,16)
\rput[l](81.25,19.38){$\comonunit$}
\rput[r](65.62,19.38){$\comonunit$}
\rput[r](27.5,0){$\monunit$}
\rput[l](47.5,31.25){$\monunit$}
\rput[l](80.62,31.25){$\monunit$}
\rput[l](81.25,0){$\monunit$}
\rput[l](44.38,0){$\monunit$}
\rput[l](39.38,19.38){$\comonunit$}
\rput(25,10.62){$\eqls$}
\end{pspicture}

